VidPlat: A Tool for Fast Crowdsourcing of Quality-of-Experience Measurements

For video or web services, it is crucial to measure user-perceived quality of experience (QoE) at scale under various video quality or page loading delays. However, fast QoE measurements remain challenging as they must elicit subjective assessment from human users. Previous work either (1) automates QoE measurements by letting crowdsourcing raters watch and rate QoE test videos or (2) dynamically prunes redundant QoE tests based on previously collected QoE measurements. Unfortunately, it is hard to combine both ideas because traditional crowdsourcing requires QoE test videos to be pre-determined before a crowdsourcing campaign begins. Thus, if researchers want to dynamically prune redundant test videos based on other test videos' QoE, they are forced to launch multiple crowdsourcing campaigns, causing extra overheads to re-calibrate or train raters every time. This paper presents VidPlat, the first open-source tool for fast and automated QoE measurements, by allowing dynamic pruning of QoE test videos within a single crowdsourcing task. VidPlat creates an indirect shim layer between researchers and the crowdsourcing platforms. It allows researchers to define a logic that dynamically determines which new test videos need more QoE ratings based on the latest QoE measurements, and it then redirects crowdsourcing raters to watch QoE test videos dynamically selected by this logic. Other than having fewer crowdsourcing campaigns, VidPlat also reduces the total number of QoE ratings by dynamically deciding when enough ratings are gathered for each test video. It is an open-source platform that future researchers can reuse and customize. We have used VidPlat in three projects (web loading, on-demand video, and online gaming). We show that VidPlat can reduce crowdsourcing cost by 31.8% - 46.0% and latency by 50.9% - 68.8%.

==> design_outline.tex <==
\section{Proposed framework of \name}

\subsection{Programming model}

Provide a code example of using \name to support dynamic assignment allocation.
Explain why it is easy to use.
\begin{itemize}
    \item Show the code example of \name. 
    \item Explain it is easy to use
    \begin{itemize}
        \item  Developers do not have to know all the assignments and the number of workers in the beginning. Developers only need to set a small set of initial assignments.
        \item It is a trivial change for the developers using \name
        \begin{itemize}
            \item Show the interactions between developers and Eyeorg/Sensei/\name
            \item Show how Eyeorg/Sensei and \name determine the assignments in the tasks. We want to show they share similar logic to determine the next assignments based on the collected QoE ratings.
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsection{Design of \name}
\begin{itemize}
    \item Unbiased QoE measurement
    \item Interface that supports multiple applications
    \item Flexible worker recruitment
    \item Rating validation
    \item logic debugging
\end{itemize}

\subsection{Set up and Conduct user study}
\begin{itemize}
    \item Developer interface
    \item Worker interface
    \item Workflow of \name
\end{itemize}


\section{Use cases}

\subsection{On-demand video streaming}
\begin{itemize}
    \item How to leverage QoE models to stream on-demand videos.
    \begin{itemize}
        \item video streaming backgrounds: a video is partitioned into chunks. those chunks are transmitted over fluctuating networks.
        \item video player decides to request a proper bitrate to maximize the QoE model.
    \end{itemize}
    \item Why we need to build QoE models frequently. Videos have different QoE models.
    \item Two baselines of scheduling QoE studies.
    \begin{itemize}
        \item baseline 1: Enumerate all combinations of quality issues.
        \item baseline 2: Two tasks: 1. Grouping similar chunks; 2. Refining the representative chunk in each group.
    \end{itemize}
    \item \name can improve the cost and latency over the baselines
    \begin{itemize}
        \item baseline 2 has to separate grouping and refining in different tasks.
        \item opportunity: when we complete a chunk's rating collection, if this chunk does not have other similar chunks, we can directly start to refine its weights.
    \end{itemize}
\end{itemize}

\subsection{Online gaming}
\begin{itemize}
    \item How to leverage QoE models to stream gaming videos.
    \begin{itemize}
        \item Users concern MTP latency and visual quality (bitrate)
        \item We need to balance FEC level (minimize MTP latency) and video bitrate.
    \end{itemize}
    \item Different gaming scenarios have different QoE models
    \item Two baselines of building QoE models.
    \begin{itemize}
        \item Baseline 1: sampling (MTP, Bitrate) with small intervals in one task.
        \item Baseline 2: sampling.
    \end{itemize}
    \item \name can improve the second baseline.
\end{itemize}

\subsection{Web services}
\begin{itemize}
    \item Use QoE models to optimize web services
    \begin{itemize}
        \item allocate computing resources across the web requests.
    \end{itemize}
    \item Different webpages have different models.
    \item Baselines of building QoE models
    \item Why \name can improve.
\end{itemize}




\section{Discussion}

\begin{itemize}
    \item what scenarios \name cannot build QoE models?
    \begin{itemize}
        \item Testing videos under different viewing environments (brightness, etc.), since we cannot control and monitor the worker's environment.
        \item Cannot allocate assignments to specific workers. cannot build per-user models. cannot model the memory effect.
    \end{itemize}

    \item Limitations on developers
    \begin{itemize}
        \item Need fast developer-provided logic/the bottleneck must be. If it is too long, we cannot let the workers wait for a long time.
    \end{itemize}
\end{itemize}

==> design_v5.tex <==
\section{Implementation}
\label{sec:impl}

In this section, we present an early implementation of \name, developed to support the programming model as outlined in \S\ref{sec:prog_model}. 
The section details how \name schedules user-study tasks to effectively minimize both the monetary cost and latency.


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{fake_graph/work_flow.pdf}
    \caption{Workflow of \name}
    \label{fig:workflow}
\end{figure}


\subsection{Workflow}

Figure~\ref{fig:workflow} illustrates the workflow of \name. 
The steps of the process are as follows:
\begin{enumerate}[leftmargin=*]
\item User-study requesters are required to specify a budget (for instance, the maximum payment for collecting a QoE rating), worker eligibility criteria (such as expertise and demographics), and the assignment generator logic, as described in \S\ref{sec:prog_model}, for \name.
\item \name employs the provided logic to produce the initial assignments or to create additional assignments based on the collected QoE ratings.
\item The worker management module handles the workers. 
This includes recruitment, retention, and release of the workers based on the assignment to rate and the quality of the workers' ratings. 
Additionally, it allocates assignments to workers to ensure unbiased QoE measurement (for more details, refer to \S\ref{subsec:impl}).
\item Upon the determination to recruit more workers by \name, it instructs the task publisher to engage with the crowdsourcing platforms at appropriate worker pricing.
\item The QoE ratings of the assignments are collected from the workers.
\item The quality controller verifies the validity of the worker ratings. 
Valid ratings are sent to the assignment generator for obtaining subsequent assignments. 
The validity of ratings is also reported to the worker management module for managing the workers (more details in~\S\ref{subsec:impl}).
\item \name repeats steps (2) through (6) until no more assignment ratings need to be collected.
\end{enumerate}
Once all the steps are completed, \name outputs the valid QoE ratings of the assignments. These can then be used to train accurate QoE models. 
Throughout the entire process, requesters do not need to concern themselves with how to operate the user study (for instance, interacting with the online workforce marketplace, or managing workers).


\subsection{Design choices}
\label{subsec:impl}

Distinct from prior crowdsourcing tools which require requesters to provide application demos prior to the user-study task start, with \name, requesters provide logic to dynamically generate the application demos during the task. 
This change presents two unique challenges:
\begin{packeditemize}
\item {\bf Challenge 1:} How can we ensure unbiased QoE measurement? 
In \name, each application demo is rated by a varying number of workers to save the cost. 
Each worker's unique working environment might introduce bias into QoE ratings. 
For instance, a worker with a low-resolution device might differentiate high- and low-quality videos~\cite{zhu2015understanding}.
\item {\bf Challenge 2:} How should the application demo generation logic interface be designed to ensure broad Internet application compatibility? 
In \name, we need to support a range of applications like video streaming and web services. 
A properly designed presentation is required for these applications to make it easy for requesters to program the logic.
\end{packeditemize}

\mypara{Unbiased QoE measurement}
We utilize {\em assignment-level randomization} to avoid bias in QoE measurement. 
In other words, an application demo should be allocated to random workers.
In \name, we need to consult the logic provided by the requester to determine a worker's assignments.
As this logic is blind to any information about the workers, it cannot make an application demo allocation decision that would eliminate potential bias.
Because if the logic only outputs one application demo, inevitably, this demo becomes the sole choice for the worker waiting for their next assignment, indicating that allocation depends on worker speed and arrival time.
To solve this issue, we instruct the logic to output as many application demos as possible, enabling us to allocate a random application demo to a worker, \ie multiple items in {\ttfamily demo\_to\_emit()} in Figure~\ref{fig:code_example_web}.

In addition to demo allocation, we need to validate the worker QoE ratings. 
This is not a trivial task because QoE measurement lacks ground-truth answers.
In \name, we do not invent new techniques, but rather adopt a combination of common practices~\cite{varvello2016eyeorg, hossfeld2014best, hossfeld2013best}.
We apply {\em golden standards}, which are control questions related to events that occur in the assignment (\eg ``did you see a resolution drop in the video?''). 
These control questions are easy to answer if workers conscientiously complete their assignments.
Moreover, we ensure workers watch the entire application demo before giving their QoE feedback by monitoring the active time of the webpage tab containing the video players.
If a worker does not watch the full video or fails to answer the control questions, we will not accept their QoE ratings.

\mypara{Assignment generator interface}
Inspired by~\cite{varvello2016eyeorg}, we use {\em videos} to present the application demos for different applications. 
For any application demo, we can acquire it by a raw video representing the application without any quality issues, further customized by a series of sequential quality change events. 
For instance, if we wish to add an extra 0.1-second MTP latency for a one-second clip in an online game video, we could slow down the playback rate of this clip by 10\% or freeze each frame within this clip. 
We detail the definitions of the data types used in logic in~\S\ref{subsec:type_definition}.
